Locating topological structures in digital images via local homology

Topological data analysis (TDA) is a rising branch in modern applied mathematics. It extracts topological structures as features of a given space and uses these features to analyze digital data. Persistent homology, one of the central tools in TDA, defines persistence barcodes to measure the changes in local topologies among deformations of topological spaces. Although local spatial changes characterize barcodes, it is hard to detect the locations of corresponding structures of barcodes due to computational limitations. The paper provides an efficient and concise way to divide the underlying space and applies the local homology of the divided system to approximate the locations of local holes in the based space. We also demonstrate this local homology framework on digital images.

==> History_and_Buff/Buff.tex <==
\begin{figure}%
  \centering
  \subfloat[A $6 \times 6$ image domain]{
  %\ytableausetup{centertableaux}
  %\ytableausetup{centertableaux}
\begin{ytableau}
*(white) & *(white) & *(white) & *(white) & *(white) & *(white)\\
*(white) & *(white) & *(white) & *(white) & *(white) & *(white)\\
*(white) & *(white) & *(white) & *(white) & *(white) & *(white)\\
*(white) & *(white) & *(white) & *(white) & *(white) & *(white)\\
*(white) & *(white) & *(white) & *(white) & *(white) & *(white)\\
*(white) & *(white) & *(white) & *(white) & *(white) & *(white)\\
  \end{ytableau}}~
   \subfloat[A $3 \times 3$ window]{
 \begin{ytableau}
*(green) & *(green) & *(green) & *(white) & *(white) & *(white)\\
*(green) & *(blue) & *(green) & *(white) & *(white) & *(white)\\
*(green) & *(green) & *(green) & *(white) & *(white) & *(white)\\
*(white) & *(white) & *(white) & *(white) & *(white) & *(white)\\
*(white) & *(white) & *(white) & *(white) & *(white) & *(white)\\
*(white) & *(white) & *(white) & *(white) & *(white) & *(white)\\
  \end{ytableau}}~
  \subfloat[The patches from (b)]{
\begin{ytableau}
*(green) & *(green) & *(green) & *(green) & *(green) & *(green)\\
*(green) & *(blue) & *(green) & *(green) & *(blue) & *(green)\\
*(green) & *(green) & *(green) & *(green) & *(green) & *(green)\\
*(green) & *(green) & *(green) & *(green) & *(green) & *(green)\\
*(green) & *(blue) & *(green) & *(green) & *(blue) & *(green)\\
*(green) & *(green) & *(green) & *(green) & *(green) & *(green)\\
  \end{ytableau}}\\
  \subfloat[A binary image]{
\begin{ytableau}
*(white) & *(white) & *(white) & *(white) & *(white) & *(white)\\
*(gray) & *(gray) & *(gray) & *(white) & *(white) & *(white)\\
*(gray) & *(white) & *(gray) & *(white) & *(gray) & *(gray)\\
*(gray) & *(white) & *(gray) & *(white) & *(gray) & *(white)\\
*(gray) & *(gray) & *(gray) & *(gray) & *(gray) & *(white)\\
*(white) & *(white) & *(white) & *(white) & *(white) & *(white)\\
  \end{ytableau}}~
  \subfloat[$R + (1,-1)$]{
  %\ytableausetup{centertableaux}
\begin{ytableau}
*(white) & *(white) & *(white) & *(white) & *(white) & *(white)\\
*(white) & *(green) & *(green) & *(green) & *(green) & *(white)\\
*(white) & *(green) & *(blue) & *(blue) & *(green) & *(white)\\
*(white) & *(green) & *(green) & *(green) & *(green) & *(white)\\
*(white) & *(white) & *(white) & *(white) & *(white) & *(white)\\
*(white) & *(white) & *(white) & *(white) & *(white) & *(white)\\
  \end{ytableau}}~
  \subfloat[$R + (2,-1)$]{
  %\ytableausetup{centertableaux}
\begin{ytableau}
*(white) & *(white) & *(white) & *(white) & *(white) & *(white)\\
*(white) & *(white) & *(green) & *(green) & *(green) & *(green)\\
*(white) & *(white) & *(green) & *(blue) & *(blue) & *(green)\\
*(white) & *(white) & *(green) & *(green) & *(green) & *(green)\\
*(white) & *(white) & *(white) & *(white) & *(white) & *(white)\\
*(white) & *(white) & *(white) & *(white) & *(white) & *(white)\\
  \end{ytableau}}
  \caption{An illustration of the sliding window technique to cover the whole region of the image domain. As in Figure \ref{Fig. Local section in images}, the green pixels represent the boundary of the sliding window.}
  \label{Fig. sliding window technique}
\end{figure}
